NESTOR: A Nested MOE-based Neural Operator for Large-Scale PDE Pre-Training

Neural operators have emerged as an efficient paradigm for solving PDEs, overcoming the limitations of traditional numerical methods and significantly improving computational efficiency. However, due to the diversity and complexity of PDE systems, existing neural operators typically rely on a single network architecture, which limits their capacity to fully capture heterogeneous features and complex system dependencies. This constraint poses a bottleneck for large-scale PDE pre-training based on neural operators. To address these challenges, we propose a large-scale PDE pre-trained neural operator based on a nested Mixture-of-Experts (MoE) framework. In particular, the image-level MoE is designed to capture global dependencies, while the token-level Sub-MoE focuses on local dependencies. Our model can selectively activate the most suitable expert networks for a given input, thereby enhancing generalization and transferability. We conduct large-scale pre-training on twelve PDE datasets from diverse sources and successfully transfer the model to downstream tasks. Extensive experiments demonstrate the effectiveness of our approach.

==> arXiv_CVPR_2026_NESTOR/preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> sec/2_Related_Works.tex <==
\section{Related Works}
\label{headings}

\subsection{Neural Operators} 
Neural operators are designed to learn mesh-free, function-space-to-function-space infinite-dimensional mappings from inputs to solution functions~\cite{lu2019deeponet}. They effectively overcome the dependence of traditional numerical solvers on mesh discretization, improving computational speed and reducing costs. Moreover, for repeated problems, a neural operator only needs to be trained once, without retraining for each new PDE instance, making it an efficient paradigm for PDE solving. To successfully apply neural operators to PDE problems, researchers have proposed several effective model architectures. For example, DeepONet~\cite{lu2019deeponet} adopts a branch–trunk architecture to realize operator learning. The Fourier Neural Operator (FNO)~\cite{li2020fourier} leverages Fourier transforms to capture non-local dependencies, thus enabling efficient PDE solutions. The Galerkin Transformer~\cite{cao2021choose} integrates self-attention mechanisms with Galerkin projection for operator learning. GNOT~\cite{hao2023gnot} combines graph neural operators with Transformers, achieving efficient modeling on irregular meshes. MPP~\cite{mccabe2023multiple} is a Transformer-based autoregressive pre-training architecture. DPOT~\cite{hao2024dpot} employs autoregressive denoising pre-training combined with Fourier attention to predict a wide range of PDE problems. Poseidon~\cite{herde2024poseidon} integrates neural operators with hybrid attention mechanisms to enable efficient and unified modeling of diverse PDEs. VITO~\cite{ovadia2024vito} integrates Vision Transformers with neural operator principles, enabling vision-based PDE solving and physical field modeling. Unisolver~\cite{zhouunisolver} employs a PDE-conditional Transformer architecture to achieve unified solving across diverse PDEs, advancing toward universal neural PDE solvers. Despite the significant progress made by neural operators, their performance still has room for improvement due to the limitations imposed by the diversity of data and tasks.



\subsection{Mixture of Experts}
The Mixture of Experts (MoE) framework is a method that expands model capacity while avoiding a significant increase in computational cost. Its core idea is to select a subset of experts among multiple expert networks through a gating mechanism ~\cite{jacobs1991adaptive}. With the development of MoE, it has been widely applied in natural language processing, computer vision, and other domains. GShard~\cite{lepikhin2020gshard} was the first to introduce the MoE structure into Transformer models, enabling efficient large-scale distributed training. Switch Transformer~\cite{fedus2022switch} scaled large language model parameters to the trillion level, significantly improving both model capacity and efficiency. V-MoE~\cite{riquelme2021scaling} applied MoE to vision Transformers and demonstrated its potential for enhancing efficiency and performance in tasks such as image recognition. Existing work primarily focuses on homogeneous experts, while research on heterogeneous~\cite{wang2024hmoe} experts is relatively limited. Homogeneous experts refer to all experts using the same network architecture, which offers simplicity in implementation, stable convergence, and ease of load balancing. However, having identical architectures limits expert diversity and, to some extent, constrains the performance of MoE. Heterogeneous expert MoE allows different experts to adopt different network architectures, avoiding redundancy in the features learned by the experts and significantly enhancing the model’s expressive power and efficiency. 


\subsection{Pre-training}
Pre-training~\cite{bengio2012deep} refers to the process of training a model on large-scale datasets to learn general knowledge that can be transferred to a variety of downstream tasks. It can significantly reduce the training cost of downstream tasks while improving generalizability. The pre-training paradigm has achieved outstanding success in natural language processing, demonstrating strong cross-task transferability, as exemplified by models such as BERT~\cite{devlin2019bert} and GPT~\cite{radford2018improving}. In computer vision, pre-training has also been widely adopted, with notable examples including the Vision Transformer (ViT)~\cite{dosovitskiy2020image} and CLIP~\cite{radford2021learning}. With the development of large-scale pre-training models, this approach has gradually been introduced into the field of PDE neural operators. Existing explorations include MPP~\cite{mccabe2023multiple}, which proposes a Transformer-based autoregressive pre-training framework capable of learning unified serialized representations across various PDE datasets and allowing cross-task modeling through transfer. DPOT~\cite{hao2024dpot} employs an autoregressive denoising strategy combined with Fourier attention to achieve efficient pre-training across multiple types of PDE problems, demonstrating cross-equation generalization at the operator level. Although these studies have successfully applied pre-training techniques to PDE neural operators, they still exhibit notable limitations in comprehensively capturing PDE systems. Therefore, there remains substantial room for further exploration of large-scale pre-training in the PDE neural operator domain.





==> sec/4_Proposed_Method.tex <==
\section{Proposed Method}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figuers/overview.pdf}
    \caption{Overview architecture. We train on twelve mixed PDE datasets, predicting the next frame based on the preceding frames. We design a nested MoE architecture: (1) the top shows the overall model architecture; (2) the bottom right illustrates the nested Sub-MoE architecture; and (3) the bottom left depicts the improved Flash Attention architecture.}
    \label{fig:overview}
\end{figure*}


We propose a nested MoE framework (NESTOR), as shown in Fig.~\ref{fig:overview}. First, the PDE input is mapped to a latent representation space~\cite{hao2024dpot}. Then, these representations are input into nested MoE modules, and a gating mechanism assigns them to different experts, each capable of learning specific features of the input. The proposed network architecture integrates frequency domain features and spatiotemporal features, addressing the diversity and complexity of PDEs at both the image and token levels, thus demonstrating strong robustness and generalization ability.




\subsection{Spatio-Temporal Encoding}
First, the input $x \in \mathbb{R}^{B \times C \times H \times W}$ 
is divided into a set of non-overlapping patches 
$X_p \in \mathbb{R}^{B \times N \times C \times P_H \times P_W}$, 
where $B$ is the batch size, $N$ is the number of patches, and $(P_H \times P_W)$ is the patch size. 
Each patch is then projected into a $D$-dimensional space, followed by the addition of positional encoding $E_\text{pos}$~\cite{dosovitskiy2020image}:
\begin{equation}
X = \text{Embedding}(X_p) + E_\text{pos} \in \mathbb{R}^{B \times N \times D},
\end{equation}
Subsequently, the obtained representation is rearranged as 
$X \in \mathbb{R}^{B \times X \times Y \times T \times C}$, 
and mapping time series to a fixed dimension to compress information in the time dimension:  
\vspace{-6pt}
\begin{equation}
Y = \sum_{t=1}^{T} W_t X_t, \quad 
Y \in \mathbb{R}^{B \times X \times Y \times C_\text{out}},
\vspace{-6pt}
\end{equation}
where $W \in \mathbb{R}^{T \times C_\text{out} \times C_\text{out}}$ is a learnable weight matrix.





\subsection{Nested Mixture-of-Experts Architecture}
A single type of network architecture is insufficient to fully capture the diverse characteristics of data. To address this, we introduce a nested MoE architecture at the operator level to enable multi-scale interactions within the PDE system. This module dynamically allocates the most appropriate expert network through a routing mechanism, allowing it to simultaneously characterize both local and global dependencies and effectively capture features in both the time and frequency domains. Here, both the image-level MoE and the token-level Sub-MoE consist of 6 non-shared experts and 1 shared expert, with the gating network activating 2 of the non-shared experts.




\subsubsection{Image-level MoE}
\textbf{Routing Strategy.} We adopt an image-level gating mechanism and employ a top-k routing strategy~\cite{shazeer2017outrageously} for expert selection. First, given the input feature $x \in \mathbb{R}^{B \times C \times H \times W}$, we apply global average pooling to obtain the image-level representation $\bar{x}_b \in \mathbb{R}^C$, where $b=1,\dots,B$.
Next, the image-level representation is fed into a learnable linear layer to produce the raw expert scores:
\begin{equation}
s_b = \bar{x}_b W^\top + b \in \mathbb{R}^N,
\end{equation}
where $W \in \mathbb{R}^{N \times C}$ is the expert weight matrix, $b \in \mathbb{R}^N$ is the bias term, and $N$ denotes the number of experts.
The raw scores are then normalized using the softmax to obtain the routing probabilities
\vspace{-6pt}
\begin{equation}
p_b = \texttt{softmax}(s_b), \quad \sum_{i=1}^{N} p_{b,i} = 1.
\vspace{-6pt}
\end{equation}
Finally, according to the top-$k$ routing strategy, the $k$ experts with the highest probabilities are selected. Let $\mathcal{I}_b$ denote the index set of the selected experts. For each selected expert $i \in \mathcal{I}_b$, the final routing weight is defined as:
\begin{equation}
w_{b,i} = \frac{p_{b,i}}{\sum_{j \in \mathcal{I}b} p{b,j}}, \quad i \in \mathcal{I}_b.
\end{equation}
\vspace{-6pt}


\noindent\textbf{Expert Design.} We select AFNO~\cite{guibas2021adaptive}~\cite{hao2024dpot} as the shared expert, responsible for capturing global low-frequency spatial features. First, the input feature $x \in \mathbb{R}^{B \times C \times H \times W}$ is Fourier transformed:
$\hat{x} = \mathcal{F}(x), \quad \hat{x} \in \mathbb{C}^{B \times H \times W \times C}$, where $\mathcal{F}(\cdot)$ is the FFT operation. Next, a complex convolution operation is performed in the frequency domain:
\vspace{-1pt}
\begin{align} 
&\hat{y}_{\mathrm{real}} = \sigma \Big( \hat{x}_{\mathrm{real}} W_1^{(r)} - \hat{x}_{\mathrm{imag}} W_1^{(i)} + b_1^{(r)} \Big),\\
&\hat{y}_{\mathrm{imag}} = \sigma \Big( \hat{x}_{\mathrm{imag}} W_1^{(r)} + \hat{x}_{\mathrm{real}} W_1^{(i)} + b_1^{(i)} \Big),
\vspace{-5pt}
\end{align}
where $\sigma$ is the activation function, $W_1^{(r)}, W_1^{(i)}$ are learnable matrices for the real and imaginary parts, respectively, and $b_1^{(r)}, b_1^{(i)}$ are bias terms. Then, an inverse Fourier transform is performed to return to the spatiotemporal representation:
\begin{equation}
y = \mathcal{F}^{-1}(\hat{y}),
\end{equation}
where $\mathcal{F}^{-1}(\cdot)$ represents the IFFT operation. Finally, a normalization layer, MLP, and residual connections are combined to obtain the output of the shared expert.

In addition, we introduce Flash Attention~\cite{dao2022flashattention} as a non-shared expert, responsible for capturing the fine-grained spatiotemporal features of the physical field. First, the input feature \(x \in \mathbb{R}^{B \times C \times H \times W}\) is reshaped into a sequence form 
\(x' \in \mathbb{R}^{B \times C \times N}\) , where $\ N$ = $H \times W$. Next, \(x'\) is normalized and linearly transformed to obtain the query (\(Q\)), key (\(K\)), and value (\(V\)) representations. The attention-weighted result is then computed as
$Z = \text{softmax}\Big(\tfrac{Q K^\top}{\sqrt{d_k}}\Big) V$, which is added to the input residual and further normalized to obtain 
\(\tilde{Z}\). Subsequently, \(\tilde{Z}\) is passed through a Sub-MoE module for linear transformation:
\begin{equation}
Y = \texttt{Sub-MoE}(\tilde{Z}).
\end{equation}
Finally, by combining residual connections and normalization layers, we obtain the output of the non-shared expert.




\subsubsection{Token-level Sub-MoE}
\textbf{Routing Strategy.} We adopt a token-level gating mechanism and employ a top-k routing strategy for expert selection. Unlike the image-level gating mechanism, the token-level gates expert scores for each individual token vector, enabling finer-grained expert selection.
% $s_{b,n} = x_{b,n} W^{\top} + b, \quad s_{b,n} \in \mathbb{R}^{M}$, where $x_{b,n} \in \mathbb{R}^{C}$ represents the $n$th token feature of the $b$th sample, $W \in \mathbb{R}^{M \times C}$ is the expert weight matrix, $b \in \mathbb{R}^{M}$ is the bias term, and $M$ is the number of experts. Afterward, the raw scores are normalized, and the $k$ expert index set $\mathcal{I}{b,n}$ with the highest scores is selected. Each token is then dynamically assigned to the selected expert for processing:
% %\vspace{-6pt} 
% \begin{equation}
% w{b,n,i} = \frac{p_{b,n,i}}{\sum_{j \in \mathcal{I}{b,n}} p{b,n,j}}, \quad i \in \mathcal{I}_{b,n}.
% %\vspace{-6pt} 
% \end{equation}
% %\vspace{-6pt} 
% where $p{b,n,i}$ is the normalized score of the $n$th token in the $b$th sample for the $i$th expert, and $w_{b,n,i}$ is the final weight assigned.


\noindent\textbf{Expert Design.} Our Sub-MoE implements the functionality of the FFN layer in Flash Attention. Both the shared and non-shared experts adopt the same network structure, which is an MLP. Normalized features are fed into the Sub-MoE, where token-level routing assigns them to the most appropriate expert for processing, extracting fine-grained feature representations. The computational process is as follows.
\begin{equation}
\texttt{ExpertMLP}(x) = W_2 \, \sigma(W_1 x + b_1) + b_2,
\end{equation}
where $W_1 \in \mathbb{R}^{C \times (rC)}$, $W_2 \in \mathbb{R}^{(rC) \times C}$, $r$ is $\text{mlp\_ratio}$, $\sigma(\cdot)$ denotes the activation function of GELU. Specifically, we first perform the first-layer linear transformation on the input feature $h = x W_1 + b_1$. Next, perform a nonlinear activation on $h$: $a = \texttt{GELU}(h)$. Finally, a second linear transformation is performed to obtain the final feature representation: $y = a W_2 + b_2$.








\subsection{Head and Loss Function}
\subsubsection{Load Balancing Loss}
In our nested MoE model, the routing mechanism assigns tokens to the most suitable experts. A balanced distribution of tokens among experts is crucial for MoE performance. When the allocation is imbalanced, some experts remain idle and fail to learn diverse features, while a few experts become overloaded, potentially causing memory bottlenecks. This can lead the model to degenerate to using only a subset of experts, failing to fully leverage the advantages of MoE~\cite{shazeer2017sparsely}. To address this issue, we introduce a load-balancing loss~\cite{shazeer2017outrageously} to encourage a more uniform distribution of tokens across experts. Here, the two load balancing losses are defined following the same pattern:
\vspace{-6pt}
\begin{equation}
\mathcal{L}_{\mathrm{aux}} = E \sum_{i=1}^E p_i \cdot f_i, 
\end{equation}
where $p_i = \frac{1}{N} \sum_{j=1}^N P_{ij}$ is the routing probability of expert $i$, $f_i = \frac{n_i}{\sum_{k=1}^E n_k}$ is the actual token assignment ratio of expert $i$, $E$ is the total number of experts, $N$ is the total number of tokens, $P_{ij}$ is the probability of token $j$ being assigned to expert $i$, and $n_i$ denotes the number of tokens assigned to expert $i$.

\subsubsection{Main Task Loss}
For our prediction task, we choose the relative error (L2RE)~\cite{li2020fourier} as the main task loss function:
\begin{equation}
\mathcal{L}_{2} = 
\tfrac{\left\| \hat{y}_i^{(c)} - y_i^{(c)} \right\|_{2}}
     {\left\| y_i^{(c)} \right\|_{2}},
\vspace{-6pt}
\end{equation}
where $y_i^{(c)}$ is the ground-truth of $i$-th sample at channel $c$, 
and $\hat{y}_i^{(c)}$ is the corresponding prediction.

\subsubsection{Total Loss}
Ultimately, our loss function consists of the main task loss and two load-balancing losses:
\begin{equation}
\mathcal{L} = \mathcal{L}_{2} + \alpha \mathcal{L}_{\mathrm{aux_1}} + \beta \mathcal{L}_{\mathrm{aux_2}},
\vspace{-3pt}
\end{equation}
where $\mathcal{L}_{2}$ denotes the main task's L2RE; $\mathcal{L}_{\mathrm{aux_1}}$ is the load balancing loss of Image-level MoE (image-level routing); $\mathcal{L}_{\mathrm{aux_2}}$ is the load balancing loss of the Image-level Sub-MoE (token-level routing); and $\alpha$ and $\beta$ are hyperparameters that control the contribution of the load balancing losses. 



